DANBO: Disentangled Articulated Neural Body Representations via Graph Neural Networks

Deep learning greatly improved the realism of animatable human models by learning geometry and appearance from collections of 3D scans, template meshes, and multi-view imagery. High-resolution models enable photo-realistic avatars but at the cost of requiring studio settings not available to end users. Our goal is to create avatars directly from raw images without relying on expensive studio setups and surface tracking. While a few such approaches exist, those have limited generalization capabilities and are prone to learning spurious (chance) correlations between irrelevant body parts, resulting in implausible deformations and missing body parts on unseen poses. We introduce a three-stage method that induces two inductive biases to better disentangled pose-dependent deformation. First, we model correlations of body parts explicitly with a graph neural network. Second, to further reduce the effect of chance correlations, we introduce localized per-bone features that use a factorized volumetric representation and a new aggregation function. We demonstrate that our model produces realistic body shapes under challenging unseen poses and shows high-quality image synthesis. Our proposed representation strikes a better trade-off between model capacity, expressiveness, and robustness than competing methods. Project website: https://lemonatsu.github.io/danbo.

==> camera_ready_todos.tex <==
\SY{TODOs:}
\begin{itemize}
    \item H36M FID/KID (main paper) \sy{Done}
    \item MonoPerfcap Qualitative results (main paper) \sy{Done}
    \item Fix missing SURREAL description. \sy{Done, I simply change fig 7. description from CMUMOCAP to Surreal}
    \item Explain why NARF is not included \sy{Done, in Exp sec, aggregation strategy}
    \item DANBO GPU requirements (supp)
    \item COAP discussion \sy{(Added, at the end of related work)}
    \item Reviewer 6 wants table 3,4 merged
    \item Reviewer 6 wants larger Figure 5 \sy{Enlarged, may modify based on space later}
    \item Reviewer 6 wants Supp. Figure 1 in the main (replace fig 2, need to blur it ) \sy{Done, need to blur it}
    \item Reviewer 6 wants to have part of Supp. Figure 3 in the main 
\end{itemize}
\SY{end of TODOs}

==> figures/experiments/old_qualitative_novelpose.tex <==
\newlength\qnphmpscale
\setlength\qnphmpscale{0.195\linewidth}
%
% qnphm{a}{ps}
% a -> first example, ps-> picked subject, pi->picked image
% note: image id is sorted by PSNR
% qnphm{a}trim: trim parameters for first example
\ifblurface
\newcommand{\qnphmpost}{_blur}
\else
\newcommand{\qnphmpost}{}
\fi
\newcommand{\qnphmpath}{static/figure/experiments/h36m_unseen/}
\newcommand{\qnphmaps}{S1/} % trim 250 275 250 125
\newcommand{\qnphmapi}{000\qnphmpost}
\newcommand{\qnphmbps}{S6/} % trim 288 325 225 100
\newcommand{\qnphmbpi}{001\qnphmpost}
\newcommand{\qnphmcps}{S9/} % trim 310 375 340 125
\newcommand{\qnphmcpi}{004\qnphmpost}
\newcommand{\qnphmdps}{S11/} % trim 310 375 340 125
\newcommand{\qnphmdpi}{004\qnphmpost}
%
%
%
\begin{figure*}[h]
\setlength{\fboxrule}{0pt}%
\parbox[t]{\qnphmpscale}{
\centering
\fbox{\includegraphics
[width=\qnphmpscale,trim=300 375 350 125,clip]
{\qnphmpath\qnphmaps GT_p\qnphmapi}
}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=288 325 225 100,clip]%
{\qnphmpath\qnphmbps GT_p\qnphmbpi}}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=310 375 340 125,clip]%
{\qnphmpath\qnphmcps GT_p\qnphmcpi}}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=260 360 420 150,clip]%
{\qnphmpath\qnphmdps GT_p\qnphmdpi}}\\%
{\small Ground Truth}
}%
\hfill%
\parbox[t]{\qnphmpscale}{
\centering % l b r t
\fbox{\includegraphics
[width=\qnphmpscale,trim=300 375 350 125,clip]%
{\qnphmpath\qnphmaps NeuralBody_p\qnphmapi}
}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=288 325 225 100,clip]%
{\qnphmpath\qnphmbps NeuralBody_p\qnphmbpi}
}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=310 375 340 125,clip]%
{\qnphmpath\qnphmcps NeuralBody_p\qnphmcpi}}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=260 360 420 150,clip]%
{\qnphmpath\qnphmdps NeuralBody_p\qnphmdpi}}\\%
{\small NeuralBody}%
}
\hfill%
\parbox[t]{\qnphmpscale}{
\centering % l b r t
\fbox{\includegraphics
[width=\qnphmpscale,trim=300 375 350 125,clip]%
{\qnphmpath\qnphmaps Anim-NeRF_p\qnphmapi}
}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=288 325 225 100,clip]%
{\qnphmpath\qnphmbps Anim-NeRF_p\qnphmbpi}
}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=310 375 340 125,clip]%
{\qnphmpath\qnphmcps Anim-NeRF_p\qnphmcpi}}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=260 360 420 150,clip]%
{\qnphmpath\qnphmdps Anim-NeRF_p\qnphmdpi}}\\%
{\small Anim-NeRF}%
}%
\hfill%
\parbox[t]{\qnphmpscale}{
\centering % l b r t
\fbox{\includegraphics
[width=\qnphmpscale,trim=300 375 350 125,clip]%
{\qnphmpath\qnphmaps A-NeRF_p\qnphmapi}
}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=288 325 225 100,clip]%
{\qnphmpath\qnphmbps A-NeRF_p\qnphmbpi}
}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=310 375 340 125,clip]%
{\qnphmpath\qnphmcps A-NeRF_p\qnphmcpi}}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=260 360 420 150,clip]%
{\qnphmpath\qnphmdps A-NeRF_p\qnphmdpi}}\\%
{\small A-NeRF}%
}
\hfill%
\parbox[t]{\qnphmpscale}{
\centering
\fbox{\includegraphics
[width=\qnphmpscale,trim=300 375 350 125,clip]%
{\qnphmpath\qnphmaps Ours_p\qnphmapi}
}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=288 325 225 100,clip]%
{\qnphmpath\qnphmbps Ours_p\qnphmbpi}
}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=310 375 340 125,clip]%
{\qnphmpath\qnphmcps Ours_p\qnphmcpi}}\\%
\fbox{\includegraphics
[width=\qnphmpscale,trim=260 360 420 150,clip]%
{\qnphmpath\qnphmdps Ours_p\qnphmdpi}}\\%
{\small  Ours}%
}%
\centering%
\caption{\textbf{Unseen pose synthesis on Human3.6M~\cite{Ionescu14b} test split}.
}
\label{fig:exp-h36m-novel-pose}
\end{figure*}

==> figures/method/voxel_retrieval_old.tex <==
\begin{figure}[t]


\centering
\includegraphics[width=0.33\linewidth]{static/figure/method/voxel_retrieval}
\caption{Voxel feature retrieval. Instead of predicting volumes with a cubic memory consumption, we predict factors along each dimension and retrieve the voxel feature by projecting $\localquery$ to the three axes and 
%do linear interpolation
linearly interpolating
%to obtain 
the feature neighboring the projected location.}
%\vspace{-3mm}
\label{fig:voxel-retrieval}
\end{figure}


==> tables/experiments/ablation_minipage_old.tex <==
%\begin{table}
\setlength{\intextsep}{0pt}%
\begin{wraptable}{r}{0.40\textwidth}
\begin{minipage}{1.0\linewidth}%
\input{tables/experiments/ablation_modules}%
\end{minipage}%
%\hfill%
\\%
\begin{minipage}{1.0\linewidth}%
\input{tables/experiments/ablation_aggregation}%
\end{minipage}%
%\hfill%
\\%
\begin{minipage}{1.0\linewidth}%
\input{tables/experiments/ablation_architecture}%
\end{minipage}%
\end{wraptable}
%\end{table}

==> tables/experiments/ablation_partdis.tex <==
\newlength\tabvolresscale
%\setlength\tabvolresscale{1.0\textwidth}
\setlength\tabvolresscale{0.4\textwidth}
\begin{table}[!t]
\setlength{\intextsep}{0pt}%
%\begin{wraptable}{r}{\tabvolresscale}
\caption{\small Ablation study of patch-based training. \textbf{NOTE: this setting is different from other ablations: we train the model for 200k, with 64+32 samples, and separated bias for GNN. Top 4 rows: novel view, Bottom 4 rows: novel poses}}
\centering
\resizebox{0.4\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
%\small
\begin{tabular}{lcc}
\toprule
 % & \multicolumn{2}{c}{A-NeRF~\cite{su2021anerf}}  \\
 %\midrule
 Volume res. &   PSNR~$\uparrow$ & SSIM~$\uparrow$   \\ 
\midrule
\rowcolor{Gray}
Ours  & 26.11 & 0.924 \\
Share  & 26.17 & 0.924 \\
\rowcolor{Gray}
Ind & 25.86 & 0.921 \\
\midrule
Ours  & 24.89 & 0.905 \\
\rowcolor{Gray}
Share  & 24.86 & 0.905 \\
Ind  & 24.68 & 0.902 \\
 \bottomrule
\end{tabular}
\label{tab:exp-ablation-res}
}
% \vspace{-2mm}
\end{table}
%\end{wraptable}


==> tables/experiments/ablation_patchbase.tex <==
\newlength\tabvolresscale
%\setlength\tabvolresscale{1.0\textwidth}
\setlength\tabvolresscale{0.4\textwidth}
\begin{table}[!t]
\setlength{\intextsep}{0pt}%
%\begin{wraptable}{r}{\tabvolresscale}
\caption{\small Ablation study of patch-based training. \textbf{NOTE: this setting is different from other ablations: we train the model for 200k, with 64+32 samples, and separated bias for GNN. Top 4 rows: novel view, Bottom 4 rows: novel poses}}
\centering
\resizebox{0.4\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
%\small
\begin{tabular}{lcc}
\toprule
 % & \multicolumn{2}{c}{A-NeRF~\cite{su2021anerf}}  \\
 %\midrule
 Volume res. &   PSNR~$\uparrow$ & SSIM~$\uparrow$   \\ 
\midrule
\rowcolor{Gray}
Ours  & 26.11 & 0.924 \\
Patch  & 25.61 & 0.918 \\
\rowcolor{Gray}
Patch w/ Percept  & 25.68 & 0.920 \\
\midrule
Ours  & 24.89 & 0.905 \\
\rowcolor{Gray}
Patch  & 24.64 & 0.903 \\
Patch w/ Percept  & 24.71 & 0.903 \\
 \bottomrule
\end{tabular}
\label{tab:exp-ablation-res}
}
% \vspace{-2mm}
\end{table}
%\end{wraptable}


==> tables/experiments/ablation_volres.tex <==
\newlength\tabvolresscale
%\setlength\tabvolresscale{1.0\textwidth}
\setlength\tabvolresscale{0.4\textwidth}
\begin{table}[!t]
\setlength{\intextsep}{0pt}%
%\begin{wraptable}{r}{\tabvolresscale}
\caption{\small Ablation study of different volume resolution. \textbf{NOTE: this setting is different from other ablations: we train the model for 200k, with 64+32 samples, and separated bias for GNN. Top 4 rows: novel view, Bottom 4 rows: novel poses}}
\centering
\resizebox{0.4\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
%\small
\begin{tabular}{lcc}
\toprule
 % & \multicolumn{2}{c}{A-NeRF~\cite{su2021anerf}}  \\
 %\midrule
 Volume res. &   PSNR~$\uparrow$ & SSIM~$\uparrow$   \\ 
\midrule
\rowcolor{Gray}
16  & 26.11 & 0.924 \\
24  & 26.05 & 0.923 \\
\rowcolor{Gray}
32  & 26.17 & 0.924 \\
40  & 26.05 & 0.924 \\
\midrule
\rowcolor{Gray}
16  & 24.89 & 0.905 \\
24  & 24.80 & 0.904 \\
\rowcolor{Gray}
32  & 24.76 & 0.904 \\
40  & 24.90 & 0.905 \\
 \bottomrule
\end{tabular}
\label{tab:exp-ablation-res}
}
% \vspace{-2mm}
\end{table}
%\end{wraptable}


==> tables/experiments/h36m_old_novelpose.tex <==
\begin{table}[!t]
\caption{\textbf{Novel-pose synthesis comparisons on Human3.6M~\cite{Ionescu14b}}. Our part-disentangled design enables \ourapproach{} to generalize better to unseen poses.}
\centering
\resizebox{0.95\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
%\small
\begin{tabular}{lcccccccccccc}
\toprule
  & \multicolumn{2}{c}{NHR\cite{wu2020nhr}} & \multicolumn{2}{c}{NT~\cite{thies2019neuraltex}} & \multicolumn{2}{c}{NeuralBody~\cite{peng2020neuralbody}}  & \multicolumn{2}{c}{Anim-NeRF~\cite{peng2021animatable}} & \multicolumn{2}{c}{A-NeRF~\cite{su2021anerf}} & \multicolumn{2}{c}{\tbf{\ourapproach{} (Ours)}} \\
 \midrule
  &   PSNR~$\uparrow$ & SSIM~$\uparrow$  &   PSNR~$\uparrow$ & SSIM~$\uparrow$ &   PSNR~$\uparrow$ & SSIM~$\uparrow$  &   PSNR~$\uparrow$ & SSIM~$\uparrow$  &   PSNR~$\uparrow$ & SSIM~$\uparrow$ &   PSNR~$\uparrow$ & SSIM~$\uparrow$ \\ 
\midrule
\rowcolor{Gray}
S1 & 21.24 & 0.877& 21.08 & 0.874& 22.10 & 0.878& 21.37 & 0.868& 22.67 & 0.883& \tbf{23.03} & \tbf{0.895}\\
S5 & 21.55 & 0.883& 21.06 & 0.879& 23.52 & 0.897& 22.29 & 0.875& 22.96 & 0.888& \tbf{23.66} & \tbf{0.903}\\
\rowcolor{Gray}
S6 & 21.14 & 0.876& 21.20 & 0.875& 23.42 & 0.892& 22.59 & 0.884& 22.77 & 0.869& \tbf{24.57} & \tbf{0.906}\\
S7 & 20.52 & 0.878& 21.15 & 0.878& 22.59 & 0.893& 22.22 & 0.878& 22.80 & 0.880& \tbf{23.08} & \tbf{0.897}\\
\rowcolor{Gray}
S8 & 19.55 & 0.876& 17.67 & 0.862& 20.94 & 0.876& 21.78 & 0.882& 21.95 & 0.886& \tbf{22.60} & \tbf{0.904}\\
S9 & 23.02 & 0.883& 23.10 & 0.883& 23.05 & 0.885& 23.73 & 0.886& 24.16 & 0.889& \tbf{24.79} & \tbf{0.904}\\
\rowcolor{Gray}
S11 & 22.94 & 0.890& 22.72 & 0.889& 23.72 & 0.884& 23.92 & 0.889& 23.40 & 0.880& \tbf{24.57} & \tbf{0.901}\\
\midrule
Avg  & 21.42 & 0.880 & 21.14 & 0.877 & 22.76 & 0.886 & 22.56 & 0.880 & 22.96 & 0.882 & \tbf{23.76} & \tbf{0.902} \\
    \bottomrule
\end{tabular}
\label{tab:exp-h36m-novel-pose}
}
% \vspace{-2mm}
\end{table}


==> tables/experiments/h36m_old_novelview.tex <==
\begin{table}[!t]
\caption{\textbf{Novel-view synthesis comparisons on Human3.6M~\cite{Ionescu14b}}. The disentangled feature enables~\ourapproach{} to achieve better performance for novel view synthesis.}
\centering
\resizebox{0.95\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
%\small
\begin{tabular}{lcccccccccccc}
\toprule
  & \multicolumn{2}{c}{NHR\cite{wu2020nhr}} & \multicolumn{2}{c}{NT~\cite{thies2019neuraltex}} & \multicolumn{2}{c}{NeuralBody~\cite{peng2020neuralbody}}  & \multicolumn{2}{c}{Anim-NeRF~\cite{peng2021animatable}} & \multicolumn{2}{c}{A-NeRF~\cite{su2021anerf}} & \multicolumn{2}{c}{\tbf{\ourapproach{} (Ours)}} \\
 \midrule
  &   PSNR~$\uparrow$ & SSIM~$\uparrow$  &   PSNR~$\uparrow$ & SSIM~$\uparrow$ &   PSNR~$\uparrow$ & SSIM~$\uparrow$  &   PSNR~$\uparrow$ & SSIM~$\uparrow$  &   PSNR~$\uparrow$ & SSIM~$\uparrow$ &   PSNR~$\uparrow$ & SSIM~$\uparrow$ \\ 
\midrule
\rowcolor{Gray}
S1 & 21.79 & 0.892& 22.04 & 0.893& 22.88 & 0.897& 22.74 & 0.896& 23.93 & 0.912& \tbf{23.95} & \tbf{0.916}\\
S5 & 21.37 & 0.892& 20.91 & 0.887& 24.61 & 0.917& 23.40 & 0.895& 24.67 & 0.919& \tbf{24.86} & \tbf{0.924}\\
\rowcolor{Gray}
S6 & 21.05 & 0.854& 21.10 & 0.855& 22.83 & 0.888& 22.85 & 0.871& 23.78 & 0.887& \tbf{24.54} & \tbf{0.903}\\
S7 & 21.11 & 0.890& 21.59 & 0.891& 23.17 & 0.915& 21.97 & 0.891& 24.40 & 0.917& \tbf{24.45} & \tbf{0.920}\\
\rowcolor{Gray}
S8 & 19.80 & 0.889& 17.69 & 0.871& 21.72 & 0.894& 22.82 & 0.900& 22.70 & 0.907& \tbf{23.36} & \tbf{0.917}\\
S9 & 23.77 & 0.898& 23.80 & 0.899& 24.29 & 0.911& 24.86 & 0.911& 25.58 & 0.916& \tbf{26.15} & \tbf{0.925}\\
\rowcolor{Gray}
S11 & 22.65 & 0.891& 22.73 & 0.892& 23.70 & 0.896& 24.76 & 0.907& 24.38 & 0.905& \tbf{25.58} & \tbf{0.917}\\
\midrule
Avg  & 21.65 & 0.887 & 21.41 & 0.884 & 23.31 & 0.903 & 23.34 & 0.896 & 24.21 & 0.909 & \tbf{24.70} & \tbf{0.917} \\
    \bottomrule
\end{tabular}
\label{tab:exp-h36m-novel-view}
}
% \vspace{-2mm}
\end{table}

==> tables/experiments/perfcap_novelpose.tex <==
\begin{table}[!t]
\caption{\textbf{Novel-pose synthesis comparisons on MonoPerfCap~\cite{xu2018monoperfcap}}. \sy{DANBO achieves better perceptual qualities on in-the-wild subjects.}}
\centering
\resizebox{0.55\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
%\small
\begin{tabular}{lcccccccc}
\toprule
  & \multicolumn{4}{c}{A-NeRF~\cite{su2021anerf}} & \multicolumn{4}{c}{Ours} \\
 \midrule
  &   PSNR~$\uparrow$ & SSIM~$\uparrow$ & KID~$\downarrow$ & LPIPS~$\downarrow$  &   PSNR~$\uparrow$ & SSIM~$\uparrow$ & KID~$\downarrow$ & LPIPS~$\downarrow$  \\ 
%\midrule
\rowcolor{Gray}
Nadia & \tbf{24.88} & \tbf{0.9313} & 0.048 & 0.115& 24.44 & 0.9210 & \tbf{0.026} & \tbf{0.111}\\
Weipeng & \tbf{22.45} & \tbf{0.8930} & 0.039 & 0.125  & 22.07 & 0.8850 & \tbf{0.024} & \tbf{0.117}\\
\midrule\rowcolor{Gray}
Avg  & \tbf{23.67} & \tbf{0.9122}  & 0.044  & 0.120 & 23.25 & 0.9030  & \tbf{0.025} & \tbf{0.114} \\

    \bottomrule
\end{tabular}
\label{tab:exp-perfcap-novelpose}
}
% \vspace{-2mm}
\end{table}
\begin{comment}
\begin{table}[!t]
\caption{\textbf{Visual quality evaluation on the MonoPerfCap~\cite{xu2018monoperfcap} testing sets \SY{Describe the outcomes. }}.}
\centering
\resizebox{0.75\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
%\small
\begin{tabular}{lcccccccccc}
\toprule
  & \multicolumn{5}{c}{A-NeRF~\cite{su2021anerf}} & \multicolumn{5}{c}{Ours} \\
 \midrule
  &   PSNR~$\uparrow$ & SSIM~$\uparrow$ & FID~$\downarrow$ & KID~$\downarrow$ & LPIPS~$\downarrow$  &   PSNR~$\uparrow$ & SSIM~$\uparrow$ & FID~$\downarrow$ & KID~$\downarrow$ & LPIPS~$\downarrow$  \\ 
%\midrule
\rowcolor{Gray}
Nadia & \tbf{24.88} & \tbf{0.9313} & 60.1 & 0.0476 & 0.1148& 24.44 & 0.9210 & \tbf{43.5} & \tbf{0.0258} & \tbf{0.1114}\\
Weipeng & \tbf{22.45} & \tbf{0.8930} & 74.7 & 0.0393 & 0.1247  & 22.07 & 0.8850 & \tbf{60.8} & \tbf{0.0240} & \tbf{0.1166}\\
\midrule\rowcolor{Gray}
Avg  & \tbf{23.67} & \tbf{0.9122} & 67.4 & 0.0435  & 0.1198 & 23.25 & 0.9030 & \tbf{52.1} & \tbf{0.0249} & \tbf{0.1140} \\

    \bottomrule
\end{tabular}
\label{tab:exp-perfcap-novelpose}
}
% \vspace{-2mm}
\end{table}
\end{comment}

